Bayesian State Estimation for Unobservable Distribution Systems via Deep Learning

The problem of state estimation for unobservable distribution systems is considered. A deep learning approach to Bayesian state estimation is proposed for real-time applications. The proposed technique consists of distribution learning of stochastic power injection, a Monte Carlo technique for the training of a deep neural network for state estimation, and a Bayesian bad-data detection and filtering algorithm. Structural characteristics of the deep neural networks are investigated. Simulations illustrate the accuracy of Bayesian state estimation for unobservable systems and demonstrate the benefit of employing a deep neural network. Numerical results show the robustness of Bayesian state estimation against modeling and estimation errors and the presence of bad and missing data. Comparing with pseudo-measurement techniques, direct Bayesian state estimation via deep learning neural network outperforms existing benchmarks.

==> model.tex <==
The distribution system is described by a graph $\mathcal{N}=\{\mathcal{V}, \mathcal{E}\}$ where $\mathcal{V}=\{1,\cdots, N\}$ is the set of buses and $\mathcal{E}$ the set of network branches.  We assume that node 1 is the slack bus representing the point of common coupling (PCC), where the distribution network is connected to the main grid.

We assume an unbalanced three phase distribution system.  The  three-phase voltage phasors at bus $i$ is a complex column vector  $x_i=[x_i^1,x_i^2, x_i^3]^\intercal $, where the superscripts are phase indices and $x_i^k=V_i^k \angle\theta_i^k$, where $V_i^k$ is the voltage magnitude and $\theta_i^k$ is the phase angle for the state variable at phase $k$ of bus $i$. The overall system state $x=[x_1,\cdots, x_N]^\intercal$ is the column vector consisting of voltage phasors at all buses.

The vector of measurements $z=[z_1,\cdots, z_M]^{\T}$ is a function of the state $x$, and measurement error $e$  modeled by

\begin{equation}
z=h(x)+e,
\end{equation}

\noindent where $h(x)$ is the measurement equation and e the additive noise. The detailed modeling is in the section VII Appendix.

The available measurements helps us to estimate the state of the power system. The system is called observable if the set of measurements in the system is adequate to determine voltage magnitude and angle at every bus of the network.
Observability analysis is a well studied problem that can be found in \cite{Monticelli:12book}. The number of measurements needed for observability depends on the measurement locations and types. When the system is not observable the traditional approach is to generate pseudo-measurements until having observability is obtained, then solving the system. It is proposed a Bayesian state estimator which does not use pseudo-measurements in this paper.


